Information Extraction from Scientific Literature for Method Recommendation

As a research community grows, more and more papers are published each year. As a result there is increasing demand for improved methods for finding relevant papers, automatically understanding the key ideas and recommending potential methods for a target problem. Despite advances in search engines, it is still hard to identify new technologies according to a researcher's need. Due to the large variety of domains and extremely limited annotated resources, there has been relatively little work on leveraging natural language processing in scientific recommendation. In this proposal, we aim at making scientific recommendations by extracting scientific terms from a large collection of scientific papers and organizing the terms into a knowledge graph. In preliminary work, we trained a scientific term extractor using a small amount of annotated data and obtained state-of-the-art performance by leveraging large amount of unannotated papers through applying multiple semi-supervised approaches. We propose to construct a knowledge graph in a way that can make minimal use of hand annotated data, using only the extracted terms, unsupervised relational signals such as co-occurrence, and structural external resources such as Wikipedia. Latent relations between scientific terms can be learned from the graph. Recommendations will be made through graph inference for both observed and unobserved relational pairs.

==> 03-Data.tex <==




% \subsection{Relation Extraction on ACL Anthology Network Dataset}
% While there is a vast literature on relation extraction, but
% past work focuses primarily on extracting relations in
% single sentences. For extracting entities from domains like scientific literature, it is very important to expand the relation boundary beyond single sentences. Consider the following example from Fig.\ref{fig:sonal}. Collectively, the three sentences states that the paper use generalized LR parsing algorithm to parse the noisy phoneme sequence, which is not expressed in either sentence alone. Due to the structural nature of scientific literature,  a document level relation analysis is necessary. Therefore, we propose a relation extraction task on cross-sentence relation extraction on top of Gupta dataset. At the same time, we expand the relation types of ScienceIE based on the following aspects:

% \begin{itemize}
% \item \textbf{Hierarchy} (within category): A scientific term can be the hyponym/hypernym or synonym of another term. For example, CRF is the synonym of Conditional Random Field and self-training is a type of semi-supervised learning, therefore semi-supervised learning is a hyponym of self-training. Similarly, a task can be a subtask of another, for example, Named Entity Recognition is a subtask of information extraction and therefore Named Entity Recognition is a hyponym of Information Extraction.
% \item \textbf{Functionality} (between categories): A Method or Material is used for a certain Task. For example,  CRF and CoNLL-2000 could be the method and dataset used for POS tagging task.
% \end{itemize}


% We plan to annotate 500 paragraphs equally distributed in different sections from 100 topically diverse scientific articles from the ACL anthology. Annotation includes scientific terms (entities) and their relations based on the described ontology, where relations can span sentence boundaries. Or annotate only relation based on the 474 abstracts in Gupta dataset. \todo{Need to be discussed}

% We propose to treat the problem of automatic detection of scientific terms and their relations as an information extraction (IE) problem, where scientific terms are analogous to entities and synonymy of terms is analogous to co-reference. Additionally, the relation extraction task is to extract entity relation triples such as (CRF, is-method-of, POS tagging), but more complicated since most of the relations are embedded cross sentences. This will allow us to build on existing algorithms and evaluation frameworks while develop novel methods to this task.
